Achieving Optimal Misclassification Proportion in Stochastic Block Model

Community detection is a fundamental statistical problem in network data analysis. Many algorithms have been proposed to tackle this problem. Most of these algorithms are not guaranteed to achieve the statistical optimality of the problem, while procedures that achieve information theoretic limits for general parameter spaces are not computationally tractable. In this paper, we present a computationally feasible two-stage method that achieves optimal statistical performance in misclassification proportion for stochastic block model under weak regularity conditions. Our two-stage procedure consists of a generic refinement step that can take a wide range of weakly consistent community detection procedures as initializer, to which the refinement stage applies and outputs a community assignment achieving optimal misclassification proportion with high probability. The practical effectiveness of the new algorithm is demonstrated by competitive numerical results.

==> algo.tex <==
%!TEX root = SBM_algo.tex

\newpage
\section{A generic refinement algorithm} \label{sec:algo}

This section is devoted to the presentation of a generic refinement algorithm and its performance guarantee for the Stochastic Block Model under a weak assumption on the availability of some relatively crude community assignment method.

Suppose we have a community detection algorithm $\sigma^0$ which is able to cluster any graph on $n-1$ nodes into $k$ categories.
Let $A_{-u}$ denote the $(n-1)\times (n-1)$ submatrix of $A$ with its $u\Th$ row and $u\Th$ column removed.
For $u\in [n]$, we define $\sigma^0_u\in \{0,1,\dots, k\}^n$ where
$\sigma^0_u(u) = 0$ and for $v\neq u$, $\sigma^0_u(v) \in [k]$ denotes the community assignment obtained by applying $\sigma^0$ on $A_{-u}$.

With the above notation, 
our refinement scheme is presented in \prettyref{algo:refine}.

The algorithm works in two consecutive steps.
The first step is conducted on a node by node basis.
For each fixed node $u$, we first leave the node out and apply the available community detection algorithm $\sigma^0$ on the remaining $n-1$ nodes and the edges among them (as summarized in the matrix $A_{-u}\in \sth{0,1}^{(n-1)\times (n-1)}$)
to obtain an initial community assignment vector $\sigma^0_u$.
For convenience, we make $\sigma^0_u$ an $n$-vector by fixing $\sigma^0_u(u) = 0$, though applying $\sigma^0$ on $A_{-u}$ does not give any community assignment for $u$.
Given $\sigma^0_u$, we estimate the connectivity matrix $B$ by taking the average numbers of edges within and between communities assigned by $\sigma^0_u$.
Given an estimate of $B$, we then determine the community assignment of the  node $u$ itself by a penalized neighbor voting method \eqref{eq:refine-nb} where we assign $u$ to the community in which it has the most number of neighbors but penalized by how large the community is.
The penalty parameter $\lambda_u$ is obtained in an adaptive way as spelled out in \eqref{eq:t-set} -- \eqref{eq:lambda-set} which utilizes the estimate of $B$. 
The choice of $\lambda_u$ differs between the cases of $k=2$ and $k\geq 3$, in observation of the different structures in the minimax risk presented in \prettyref{thm:minimax}.
Once we obtain the community assignment for $u$, we organize the assignment for all $n$ vertices into an $n$-vector $\wh\sigma_u$.
Once we have conducted the above procedure for each of the $n$ nodes, we obtain $n$ vectors $\wh\sigma_u\in [k]^n$, $u=1,\dots, n$, and turn to the second step of the algorithm.
The basic idea is to obtain a unified community assignment by assembling $\{\wh\sigma_u(u):u\in [n] \}$ and the immediate difficulty we encounter is that each $\wh\sigma_u$ is only determined up to a permutation of the community labels. 
Thus, the second step aims to find the right permutations by \eqref{eq:consensus} before we assemble the $\wh\sigma_u(u)$'s.
We call this step ``consensus'' since we are essentially looking for a consensus on the community labels for $n$ possibly different community assignments, under the assumption that all of them are close to the ground truth up to some permutation.

The core of the refinement scheme lies in the penalized neighbor voting \eqref{eq:refine-nb} and the data-dependent choice of the penalty parameter \eqref{eq:t-set} -- \eqref{eq:lambda-set}.
The consensus step is a necessary extra step to align the community labels of the $\wh\sigma_u(u)$'s and itself does not improve the accuracy of the group assignment. 



\begin{algorithm}[!bth]
	\SetAlgoLined
\caption{A generic refinement scheme for community detection 
\label{algo:refine}}
% {\bf Input:} 
\KwIn{
Adjacency matrix $A\in \sth{0,1}^{n\times n}$,\\
~~~~~~~~~~~~number of communities $k$,\\
~~~~~~~~~~~~initial community detection method $\sigma^0$.
% number of communities $k$, tuning parameters $t$ and $\lambda$.
}

% {\bf Output:} 
\KwOut{
Community assignment $\wh\sigma$.
}

% {\bf Procedure:}
% \smallskip
% {\bf Coloring:}\\
% \nl For each edge in $A$, we independently label it red or blue with equal probability $\frac{1}{2}$.\\
% Denote $A^r$ the adjacency matrix resulting from all the red edges\;

\smallskip
{\bf Penalized neighbor voting:}\\
\nl \For{$u = 1$ \KwTo $n$}{
\nl Apply $\sigma^0$ on $A_{-u}$ to obtain $\sigma_u^0(v)$ for all $v\neq u$ and let $\sigma^0_u(u) = 0$\;
\nl Define $\wt{\mathcal{C}}_i^u = \sth{v: \sigma^0_u(v) = i}$ for all $i\in [k]$;
let $\wt\calE_i^u$ be the set of edges within $\wt{\mathcal{C}}_i^u$, and $\wt\calE_{ij}^u$ the set of edges between $\wt{\mathcal{C}}_i^u$ and $\wt{\mathcal{C}}_j^u$ when $i\neq j$\;
\nl Define
% For $g(x) = \frac{2x}{1+x}$, define
\begin{align}
	\label{eq:B-est}
\wh{B}_{ii}^u = \frac{|\wt\calE_i^u|}{\frac{1}{2}|\wt\calC_i^u|(|\wt\calC_i^u|-1) },
% g\pth{\frac{\wt{B}_i^u}{\frac{1}{2}|\wt{\mathcal{C}}_i^u|(|\wt{\mathcal{C}}_i^u|-1) - \wt{R}_i^u}}, 
\quad 
\wh{B}_{ij}^u = 
\frac{|\wt\calE_{ij}^u|}{|\wt\calC_i^u||\wt\calC_j^u|},
% g\pth{\frac{\wt{B}_{ij}^u}{|\wt{\mathcal{C}}_i^u||\wt{\mathcal{C}}_j^u| - \wt{R}_{ij}^u}},
\quad
\forall i\neq j\in [k],
\end{align}
and let 
\begin{align}
	\label{eq:ab-esti}
\wh{a}_u = n\min_{i\in [k]} \wh{B}_{ii}^u 
\quad \mbox{and} \quad
\wh{b}_u = n\max_{i\neq j\in [k]} \wh{B}_{ij}^u.
\end{align}

\nl Define $\wh\sigma_u: [n]\to [k]^n$ by setting $\wh\sigma_u(v)=\sigma^0_u(v)$ for all $v\neq u$ and 
\begin{align}
\label{eq:refine-nb}
\wh\sigma_u(u) = \argmax_{l\in [k]} \sum_{\sigma^0_u(v) = l} A_{uv} - \lambda_u \sum_{v\in [n]} \indc{\sigma^0_u(v)= l}
\end{align}
where for
\begin{align}
\label{eq:t-set}
t_u = \frac{1}{2}\log
{\frac{\wh{a}_u(1 - \wh{b}_u/n)}{\wh{b}_u(1 - \wh{a}_u/n)}},
\end{align}
we define
\begin{equation}
	\label{eq:lambda-set}
\lambda_u = 
\begin{cases}
-\frac{1}{2t_u}\log\pth{\frac{\frac{\wh{a}_u}{n}e^{-t_u}+1 -\frac{\wh{a}_u}{n}}{\frac{\wh{b}_u}{n}e^{t_u}+1 -\frac{\wh{b}_u}{n}}},
& \text{if}~k = 2; \\
-\frac{1}{t_u}\log\pth{\frac{\wh{a}_u}{n}e^{-t_u}+1 -\frac{\wh{a}_u}{n}}, 
& \text{if}~ k\geq 3.	
\end{cases}
\end{equation}

}

% \nl \emph{Neighbor Voting}. For each $i\in [n]$, let $\wh\sigma_i(j) = \sigma^0_i(j)$ for all $j\neq i$ and
% 
% \nb{is there a better way of writing it?}

{\bf Consensus:}\\

\nl 
Define $\wh\sigma(1) = \wh\sigma_1(1)$.
For $u=2,\dots, n$, 
define 
\begin{align}
\label{eq:consensus}
\wh\sigma(u) = \argmax_{l\in [k]} 
\left|\{v:\wh\sigma_1(v) = l\} \cap \{v: \wh\sigma_u(v) = \wh\sigma_u(u)\} \right|.
\end{align}
% \nb{double check if adjustment is needed here, perhaps a better name}
\end{algorithm}

In what follows, we show the refinement works well the initial community assignments are reasonable good, which is quantified by the following condition.
% In the rest of this section, we assume the availability of such initial community assignments. \nb{pointer to initialization section}
The investigation on what community detection methods can satisfy the condition is deferred to \prettyref{sec:init}.

\begin{condition}
\label{cond:init}
There exist constants $C_0, \delta > 0$ and a positive sequence $\gamma = \gamma_n$ 
% and a permutation $\pi_u:[k]\to [k]$ 
such that for a parameter space $\Theta$
% for each $u\in [n]$ 
\begin{align}
\inf_{(B,\sigma)\in \Theta}
\min_{u\in [n]} 
\Prob\sth{\loss(\sigma,\sigma^0_u)\leq \gamma_n} \geq 1 - C_0 n^{-(1+\delta)}.
\end{align}
\end{condition}
% \nb{for uniformity, shall we rewrite it as
% \begin{align*}
% \inf_{(B,\sigma)\in \Theta}
% \min_{u\in [n]} 
% 	\Prob_{B,\sigma}\sth{\loss(\sigma,\sigma^0_u)\leq \gamma_n} \geq 1 - C n^{-(1+\delta)}
% \end{align*}
% where $\Theta = \Theta(n,k,a,b,\beta;\alpha)$?
% }

Under \prettyref{cond:init}, we have the following upper bounds regarding the performance of the proposed refinement scheme.

\begin{theorem}
	\label{thm:upper}
% Consider parameter space $\Theta = \Theta_0(n,k,a,b)$.
Suppose as $n\to\infty$, 
% \begin{align}
$\frac{(a-b)^2}{ak} \to \infty$
\nb{also need $k\leq O(\frac{n}{\log{n}})$ for the next condition to make sense}
% \end{align}
and
there is a sequence  
\begin{align}
\label{eq:gamma-cond-1}
\gamma = \gamma_n = O\pth{\frac{1}{k\log k}}
% k \gamma \log{1\over \gamma} = O(1),
\end{align}
such that \prettyref{cond:init} holds for $\Theta = \Theta_0(n,k,a,b,\beta)$.
% with this sequence $\gamma_n$. 
Then
there is a sequence $\eta_n\to 0$ such that
\begin{equation}
	\label{eq:upper-bound}
\begin{aligned}
& \sup_{(B,\sigma)\in \Theta}\Prob_{B,\sigma}\sth{
\loss(\sigma, \wh{\sigma}) \geq
\exp\pth{-(1-\eta_n) \frac{n I^*}{2}}
% \sum_{i=1}^{k-1} \exp\sth{-(1-\eta_n)n_{(i)} I^*}
} \to 0,  & \quad \mbox{if $k = 2$},\\
& \sup_{(B,\sigma)\in \Theta}\Prob_{B,\sigma}\sth{
\loss(\sigma, \wh{\sigma}) \geq
(k-1) \exp\pth{-(1-\eta_n) \frac{n I^*}{\beta k}}
% \sum_{i=1}^{k-1} \exp\sth{-(1-\eta_n)n_{(i)} I^*}
} \to 0, & \quad \mbox{if $k \geq 3$},
\end{aligned}
\end{equation}
% \begin{eqnarray*}
% \sup_{(B,\sigma)\in \Theta}\Prob_{B,\sigma}\sth{
% \loss(\sigma, \wh{\sigma}) \geq
% (k-1)\exp\pth{-(1-\eta_n) \frac{n I^*}{k}}
% } \to 0
% \end{eqnarray*}
where $I^*$ is defined as in \eqref{eq:I}.

If in addition we have
\begin{align}
	\label{eq:gamma-cond-2}
\gamma  = o\pth{\frac{a-b}{ak}}
\end{align}
and \prettyref{cond:init} holds for $\Theta = \Theta(n,k,a,b,\lambda,\beta;\alpha)$, then the conclusion in \eqref{eq:upper-bound} continues to hold for $\Theta = \Theta(n,k,a,b,\lambda,\beta;\alpha)$.
\end{theorem}


% \begin{theorem}
% 	\label{thm:upper}
% 	% \nb{to be carefully re-written}
% % Let $A\in \sth{0,1}^{n\times n}$ be a realization of a SBM in $\Theta(n,k,a,b,\beta)$ as defined in \eqref{eq:para-space}. 
% Consider parameter space $\Theta = \Theta(n,k,a,b,\lambda,\beta;\alpha)$.
% Suppose as $n\to\infty$, $\frac{(a-b)^2}{ak} \to \infty$ and there is a sequence 
% % $\gamma = \gamma_n$ such that 
% \begin{align}
% 	\label{eq:est-cond-new}
% % \frac{(a-b)^2}{ak} \to \infty, \quad
% \gamma = \gamma_n  = O\pth{\frac{1}{k\log k}}
% \quad \mbox{and} \quad
% \gamma  = o\pth{\frac{a-b}{ak}}
% \end{align}
% such that \prettyref{cond:init} holds for $\Theta$.
%  % with this sequence $\gamma_n$. 
% Then
% there is a sequence $\eta_n\to 0$ such that
% \begin{eqnarray*}
% & \sup_{(B,\sigma)\in \Theta}\Prob_{B,\sigma}\sth{
% \loss(\sigma, \wh{\sigma}) \geq
% \exp\pth{-(1-\eta_n) \frac{n I^*}{2}}
% % \sum_{i=1}^{k-1} \exp\sth{-(1-\eta_n)n_{(i)} I^*}
% } \to 0,  & \quad \mbox{if $k = 2$},\\
% & \sup_{(B,\sigma)\in \Theta}\Prob_{B,\sigma}\sth{
% \loss(\sigma, \wh{\sigma}) \geq
% (k-1) \exp\pth{-(1-\eta_n) \frac{n I^*}{\beta k}}
% % \sum_{i=1}^{k-1} \exp\sth{-(1-\eta_n)n_{(i)} I^*}
% } \to 0, & \quad \mbox{if $k \geq 3$},
% \end{eqnarray*}
% where $I^*$ is defined as in \eqref{eq:I}.
% % \begin{align}
% % \label{eq:I}
% % I^* = -\log\pth{\pth{1-\frac{a}{n}}\pth{1-\frac{b}{n}} + \frac{a}{n}\frac{b}{n} + 2\sqrt{\pth{1-\frac{a}{n}}\pth{1-\frac{b}{n}} \frac{a}{n}\frac{b}{n}}}.
% % \end{align}
% \end{theorem}




==> init.tex <==
%!TEX root = SBM_algo.tex

% \newpage
\section{Initialization}
\label{sec:init}

In this section, we present algorithms that give consistent initial label estimators. Since the population matrix $P=\mathbb{E}[A]$ is of rank $k$. We may first reduce the dimension of the data and then apply some clustering algorithm. This is recognized as spectral clustering \citep{von2007tutorial}. One can either apply spectral clustering on the adjacency matrix directly or on the associated graph Laplacian, and the later is known as normalized spectral clustering. Though there are some debates and studies on which of the two is the better one (see, for example, \cite{von2008consistency, sarkar2013role}), as an initialization step, their performances are basically similar.

Let us use $d_u=\sum_{v\in[n]}A_{uv}$ to denote the degree of the $u\Th$ node. Then the graph Laplacian operator $L:A\mapsto L(A)$ is defined as $[L(A)]_{uv}=d_u^{-1/2}d_v^{-1/2}A_{uv}$. The performance of spectral clustering and normalized spectral clustering critically depends on the bounds $\opnorm{A-P}$ and $\opnorm{L(A)-L(P)}$. However, as pointed out by \cite{chin15} and \cite{le2015sparse}, the matrices $A$ and $L(A)$ are not good estimators of $P$ and $L(P)$ under the operator norm when the graph is sparse. Regularization is necessary for spectral methods to perform well in a sparse regime.
Define the operator $T_{\tau}: A\mapsto T_{\tau}(A)$ by zeroing out the $u\Th$ row and column of $A$ when $d_u\geq\tau$. It is argued in \cite{chin15} that by removing those high-degree nodes, $T_{\tau}(A)$ has better convergence properties. Regularization for graph Laplacian goes back to \cite{amini13} and its theoretical properties are studied by \cite{joseph2013impact, le2015sparse}. Define $A_{\tau}=A+\frac{\tau}{n}\mathbf{1}\mathbf{1}^T$. Then, \cite{amini13} propose to use $L(A_{\tau})$ for normalized spectral clustering.

The spectral algorithm is described as follows:
\begin{enumerate}
\item Apply singular value decomposition (SVD) to the matrix $T_{\tau}(A)$ or $L(A_{\tau})$. Let $\wh{U}\in\mathbb{R}^{n\times k}$ to be the singular matrix of the $k$ leading components.
\item Apply Algorithm \ref{algo:greedy} to the matrix $\wh{U}$.
\end{enumerate}

We propose the following greedy algorithm (Algorithm \ref{algo:greedy}) to do clustering on the matrix $\wh{U}$.
\begin{algorithm}[!bth]
	\SetAlgoLined
\caption{A greedy method for clustering 
\label{algo:greedy}}
% {\bf Input:} 
\KwIn{
Data matrix $\wh{U}\in \mathbb{R}^{n\times k}$,\\
~~~~~~~~~~~~number of communities $k$,\\
~~~~~~~~~~~~critical radius $r=\sqrt{\frac{2k}{\beta n}}$.
% number of communities $k$, tuning parameters $t$ and $\lambda$.
}

% {\bf Output:} 
\KwOut{
Community assignment $\wh\sigma$.
}

% {\bf Procedure:}
\smallskip
\nl Set $S=[n]$\;

\smallskip
\nl \For{$i = 1$ \KwTo $k$}{
\nl Let $t_i=\arg\max_{u\in S}\left|\left\{v\in S:\norm{\wh{U}_{v*}-\wh{U}_{u*}}<\frac{r}{6}\right\}\right|$\;
\nl Set $\wh{\mathcal{C}}_i=\left\{v\in S: \norm{\wh{U}_{v*}-\wh{U}_{t_i*}}<\frac{r}{6}\right\}$\;
\nl Label $\wh{\sigma}(u)=i$ for all $u\in\wh{\mathcal{C}}_i$\;
\nl Update $S\leftarrow S\backslash\wh{\mathcal{C}}_i$.
}
\smallskip
\nl If $S\neq\varnothing$, arbitrarily assign labels to $S$.
\end{algorithm}
It can be checked that Algorithm \ref{algo:greedy} runs in polynomial time. In contrast, the traditional k-means algorithm used in spectral clustering is NP-hard \citep{aloise2009np,mahajan2009planar}. Though \cite{lei14} applies a $(1+\epsilon)$-approximate k-means clustering algorithm by \cite{kumar2004simple} to overcome this difficulty, the complexity bound in \cite{kumar2004simple} suggests that the smallest $\epsilon$ should be at the same order of $k$, which leads to inferior statistical bounds. The greedy algorithm we propose in Algorithm \ref{algo:greedy} takes advantage of the fact that the population centers of SBM are separated from each other, thus avoiding the hardness of clustering.

The performance of the spectral method is stated without assuming SBM. We define the quantity $p_{\max}=\max_{u,v\in[n]}P_{uv}$ and $\lambda_k=\lambda_k(P)$. Intuitively speaking, $p_{\max}$ controls the variance and $\lambda_k$ is the eigen-gap.


\begin{theorem}\label{thm:ini1}
Assume
\begin{equation}
\frac{k(np_{\max}+1)}{\lambda_k^2}\leq c,\label{eq:assume}
\end{equation}
for some sufficiently small $c\in (0,1)$. Let $\wh{\sigma}$ be output from the unnormalized spectral clustering algorithm with $\tau=C_1(np_{\max}+1)$ for some sufficiently large $C_1>0$. For any constant $C'>0$, there exists some $C>0$ such that
$$\ell(\wh{\sigma},\sigma)\leq C\frac{np_{\max}+1}{\lambda_k^2},$$
with probability at least $1-n^{-C'}$.
\end{theorem}

\begin{remark}
Theorem \ref{thm:ini1} improves the error bound for spectral clustering in \cite{lei14}. While \cite{lei14} only works for the dense regime, our result works for both dense and sparse regimes. The result close to ours is by \cite{chin15}, but their clustering step is different from Algorithm \ref{algo:greedy}. Moreover, the result of Theorem \ref{thm:ini1} holds with probability $1-n^{-C'}$ for an arbitrary large $C'$, which is critical because the initialization step needs to satisfy Condition 1 for the subsequent refinement step to work. On the other hand, the bound in \cite{chin15} is stated with probability $1-o(1)$.
\end{remark}

\begin{theorem}\label{thm:ini2}
Assume
\begin{equation}
\frac{k(np_{\max}+1)\log(np_{\max}+1)}{\lambda_k^2} \leq c,\label{eq:assume2}
\end{equation}
for some sufficiently small $c\in(0,1)$. Consider normalized spectral clustering with $\tau=np_{\max}+1$. Then, for any constant $C'>0$, there exists some $C>0$ such that
$$\ell(\wh{\sigma},\sigma)\leq C\frac{(np_{\max}+1)\log(np_{\max}+1)}{\lambda_k^2},$$
with probability at least $1-n^{-C'}$.
\end{theorem}

\begin{remark}
Theorem \ref{thm:ini2} characterizes the misclassification rate of regularized normalized spectral clustering. The result is valid for both sparse and dense regime. A slightly different regularization of normalized spectral clustering is studied by \cite{qin2013regularized} only for the dense regime. Moreover, our result also improves the that of \cite{le2015sparse} due to our better bound on $\opnorm{L(A_{\tau})-L(P_{\tau})}$ in Lemma \ref{lem:sp2}. We conjecture that the $\log(np_{\max}+1)$ factor in both the assumption and the bound can be removed.
\end{remark}

Note that Theorem \ref{thm:ini1} and Theorem \ref{thm:ini2} are stated in terms of the quantities $p_{\max}$ and $\lambda_k$. We may specialize the results into the parameter spaces defined in (\ref{eq:para-space0}) and (\ref{eq:para-space}). For both spaces, $p_{\max}\lesssim a/n$. Moreover, $\lambda_k$ has an explicit lower bound in $\Theta_0(n,k,a,b,\beta)$.
\begin{proposition}\label{prop:eigen}
For SBM in the space $\Theta_0(n,k,a,b,\beta)$, we have $\lambda_k\geq \frac{a-b}{\beta k}$.
\end{proposition}
On the other hand, for the parameter space $\Theta(n,k,a,b,\lambda,\beta;\alpha)$, there is generally no explicit bound for $\lambda_k$ in terms of $a,b,k,\beta$. We simply lower bound it by $\lambda$. Combining with Theorem \ref{thm:upper}, we obtain the following convergence rates for community detection in SBM.

\begin{corollary}\label{cor:upper1}
Consider the generic refinement scheme initialized by $\sigma^0$ with unnormalized spectral clustering. For SBM in $\Theta_0(n,k,a,b,\beta)$ satisfying $\frac{ak^3\log k}{(a-b)^2}=o(1)$, the conclusion of Theorem ??? holds. For SBM in $\Theta(n,k,a,b,\lambda,\beta;\alpha)$ satisfying $\frac{ak(\log k+a/(a-b))}{\lambda^2}=o(1)$, the conclusion of Theorem \ref{thm:upper} holds.
\end{corollary}

\begin{corollary}\label{cor:upper2}
Consider the generic refinement scheme initialized by $\sigma^0$ with normalized spectral clustering. For SBM in $\Theta_0(n,k,a,b,\beta)$ satisfying $\frac{ak^3\log k\log a}{(a-b)^2}=o(1)$, the conclusion of Theorem ??? holds. For SBM in $\Theta(n,k,a,b,\lambda,\beta;\alpha)$ satisfying $\frac{ak\log a(\log k+a/(a-b))}{\lambda^2}=o(1)$, the conclusion of Theorem \ref{thm:upper} holds.
\end{corollary}

\begin{remark}
The above results which depend on various forms of spectral clustering requires to set the regularization parameter $\tau$ to the order of $np_{\max}+1\asymp a$. In fact, the results of Theorem \ref{thm:ini1} and Theorem \ref{thm:ini2} work for all $\tau\geq C(np_{\max}+1)\geq C_1a$ in order to get the misclassfication rate $\tau/\lambda_k^2$ and $\tau\log\tau/\lambda_k^2$, respectively. Thus, a data-driven choice for $\tau$ is $\frac{Ck^2}{n}\sum_{u,v\in[n]}A_{uv}$, which results in a extra $k^2$ factor in the misclassfication rate. This is practical because $k$ is usually bounded or very small in real data.
\end{remark}

\begin{remark}
Corollary \ref{cor:upper1} says that community detection using Algorithm \ref{algo:refine} initialized by unnormalized spectral clustering achieves the minimax rate uniformly over the parameter space $\Theta_0(n,k,a,b,\beta)$ as long as $\frac{ak^3\log k\log a}{(a-b)^2}=o(1)$. When $k=O(1)$, the condition reduces to $\frac{a}{(a-b)^2}=o(1)$, which is proved to be the sufficient and necessary condition for weak consistency by \cite{mossel2012stochastic, mossel2013proof}.
\end{remark}

\begin{remark}
The conditions in
both Corollary  \ref{cor:upper1} and Corollary  \ref{cor:upper2} can be weakened if the values of $a$ and $b$ are known. In particular, the parameter estimation step (\ref{eq:ab-esti}) in Algorithm \ref{algo:refine}. Then, when the unnormalized spectral clustering is used in initialization, the minimax rates are achieved as long as $\frac{ak^3}{(a-b)^2}=o(1)$ for $\Theta_0(n,k,a,b,\beta)$ and $\frac{ak}{\lambda^2}=o(1)$ for $\Theta(n,k,a,b,\lambda,\beta;\alpha)$. When the normalized spectral clustering is used in initialization, the minimax rates are achieved as long as $\frac{ak^3\log a}{(a-b)^2}=o(1)$ for $\Theta_0(n,k,a,b,\beta)$ and $\frac{ak\log a}{\lambda^2}=o(1)$ for $\Theta(n,k,a,b,\lambda,\beta;\alpha)$. 
\end{remark}



